Contention resolution on a restrained channel

We examine deterministic broadcasting on multiple-access channels for a scenario when packets are injected continuously by an adversary to the buffers of the devices at rate $\rho$ packages per round. The aim is to maintain system stability, that is, bounded queues. In contrast to previous work we assume that there is a strict limit of available power, defined as the total number of stations allowed to transmit or listen to the channel at a given time, that can never be exceeded. We study how this constraint influences the quality of services with particular focus on stability. We show that in the regime of deterministic algorithms, the significance of energy restriction depends strongly on communication capabilities of broadcasting protocols. For the adaptive and full-sensing protocols, wherein stations may substantially adopt their behavior to the injection pattern, one can construct efficient algorithms using very small amounts of power without sacrificing throughput or stability of the system. In particular, we construct constant-energy adaptive and full sensing protocols stable for $\rho=1$ and any $\rho<1$, respectively, even for worst case (adversarial) injection patterns. Surprisingly, for the case of acknowledgment based algorithms that cannot adopt to the situation on the channel (i.e., their transmitting pattern is fixed in advance), limiting power leads to reducing the throughput. That is, for this class of protocols in order to preserve stability we need to reduce injection rate significantly. We support our theoretical analysis by simulation results of algorithms constructed in the paper. We depict how they work for systems of moderate, realistic sizes. We also provide a comprehensive simulation to compare our algorithms with backoff algorithms, which are common in real-world implementations, in terms of queue sizes and energy consumption.

==> selector-constructive.tex <==



\section{Construction of selector in polynomial time}

We first describe two major components: dispersers and superimposed codes.

\noindent
{\bf Dispersers.}
A bipartite graph~$H=(V,W,E)$, with set $V$ of inputs
and set $W$ of outputs and set~$E$ of edges, 
is a \textit{$(n,\ell,d,\delta,\ep)$-disperser} 
if it has the following three properties:
%\begin{quote}
%\begin{quote}
\begin{itemize}
\item%[\sf Sizes:]
$|V|=n$ and $|W|=\ell d/\delta$;

\item%[\sf Regularity:] 
each $v\in V$ has $d$ neighbors;
%$H$ is $d$-left-regular.

\item%[\sf Dispersion:]
for each $A\subseteq V$ such that $|A|\ge \ell$,
the set of neighbors of $A$ is of size at least $(1-\ep)|W|$.
\end{itemize}
%\end{quote}
%\end{quote}
%Let graph $G=(V,W,E)$, where $|V|=n$, $|W|=\Theta((k-r+1)d/\delta)$,
%be a $(k-r+1,d,\ep)$-disperser, for some numbers $d$ and $\delta$.
%An explicit construction of such graphs, that is, 
%in time polynomial in~$n$, was given by
Ta-Shma, Umans and Zuckerman~\cite{TUZ} showed how to
construct, in time polynomial in~$n$, 
an $(n,\ell,d,\delta,\ep)$-disperser for any $\ell\le n$, some $\delta=O(\log^3 n)$
and $d=O(\text{polylog }n)$.
% is a bound on the left-degrees. 
%The value $\log\delta$ is called the {\em entropy loss} of the disperser.

\noindent
{\bf Superimposed codes.}
A set of $b$ binary codewords of length $a$, 
represented as columns of an $a\times b$ binary array,
is a \textit{$d$-disjunct} {\em superimposed code}, if it
satisfies the following property:
no boolean sum of columns in any set~$D$ of $d$ columns can cover
a column not in~$D$.
Alternatively, if codewords are representing subsets of $[a]$, then $d$-disjunctness means
that no union of up to~$d$ sets in any family of sets~$D$ could cover a set
outside~$D$.
%
Kautz and Singleton~\cite{KS} proposed a $d$-disjunct superimposed codes for $a=O(d^2 \log^2 b)$,
which could be constructed in polynomial time. 
%A book by Du and Hwang~\cite{DH} provides a contemporary
%exposition of superimposed coding and its relevance to
%nonadaptive group testing.

\noindent
{\bf Polynomial construction of light selectors.}
We show how to construct $k$-light $(n,\omega)$-selectors of length
%$\cO(\min \big[ \, n,\frac{k^2}{k-r+1} \text{ polylog }n\, \big] )$, for
%\textit{any} configuration of parameters $r\le k\le n$,
$m = O\left (\omega \text{ polylog } n\right )$ for $k \geq \frac{n}{\omega}$  and  
$m = O\left (\frac{n}{k} \text{ polylog } n\right )$  for  $k < \frac{n}{\omega}$,
in time polynomial in~$n$.
This is equivalent to constructing $k$-light $(n,\omega)$-selectors of length
%$\cO(\min \big[ \, n,\frac{k^2}{k-r+1} \text{ polylog }n\, \big] )$, for
%\textit{any} configuration of parameters $r\le k\le n$,
$m = O\left ((\omega+n/k) \text{ polylog } n\right )$ 
in time polynomial in~$n$.
The construction combines specific dispersers with superimposed codes.
%
%If $r\le 3k/4$ then we can use the construction of an
%$(n,k,3k/4)$-selector given by Indyk~\cite{Ind}.
%Assume that $r>3k/4$.
Let $0<\ep<1/2$ be a constant.
%
Let $G=(V,W,E)$ be an $(n,\omega/4,d,\delta,\ep)$-disperser for some $\delta=O(\log^3 n)$
and $d=O(\text{polylog }n)$, constructed in time polynomial in $n$, c.f., Ta-Shma, Umans and Zuckerman~\cite{TUZ}.
%
%where $|V|=n$, $|W|=\Theta((k-r+1)d/\delta)$,
%be a $(k-r+1,d,\ep)$-disperser, for some numbers $d$ and $\delta$.
%
Let $\cM=\{M_1,\ldots,M_a\}$ be the rows of the $c\delta$-disjunct 
superimposed code array of $n$ columns, for $a=O((c\delta)^2 \log^2 n)$,
constructed in time polynomial in $n$, c.f., Kautz and Singleton~\cite{KS};
here $\delta$ is the parameter from the disperser~$G$ and $c>0$ is a sufficiently large constant.
W.l.o.g. we could uniquely identify an $i$th of the $n$ columns of the superimposed code with
a corresponding $i$th node in~$V$.
%an explicit 
%$(n,c\delta\frac{k}{k-r+1})$-strongly-selective family, 
%for a sufficiently large constant $c>0$ that will be fixed later, 
%of size 
%$m=\cO(\min \big[ \, n,\delta^2(\frac{k}{k-r+1})^2\log^2
%n\,\big])$,
%as constructed by Kautz and Singleton~\cite{KS}.

For a constant integer $c$ we define a 
$k$-light $(n,\omega)$-selector $\cS(n,\omega,k,c)$ of length
$m\le \min\{n,a|W|\alpha\}$, for some $\alpha$ to be defined later, which consists of sets $S_i$, 
for $1\le i\le m$.
Consider two cases. In the case of $n\le m|W|\alpha$, we define $S_i=\{i\}$.
%take the singleton 
%containing only the $i$-th element of~$V$ as~$F(i)$.
In the case of $n> a|W|\alpha$, we first define sets $F_j$ as follows:
for $j=xa+y\le a|W|$, where $x,y$ are non-negative integers 
satisfying $x+y>0$, $F_j$ contains all the nodes $v\in V$ 
such that $v$ is a neighbor of the $x$-th node in~$W$ and $v\in M_y$;
i.e., $F_{x\cdot a+y} = M_y\cap N_G(x)$.
Next, we split every $F_j$ into $\lceil |F_j|/k \rceil$ subsets $S$ of size at most $k$ each,
and add them as elements of the selector $\cS(n,\omega,k,c)$.
Note that each set $S_i$ from $\cS(n,\omega,k,c)$ corresponds to some
set $F_j$ from which it resulted by the splitting operation; we say that $F_j$ is a parent of $S_i$ and
$S_i$ is a child of $F_j$.
In this view, parameter $\alpha$ in the upper bound $m\le a|W|\alpha$ could be interpreted as
an amortized number of children of a set $F_j$. We will show in the proof of the following theorem that
$\alpha \le \frac{nd \cdot (c\delta)^2 \log^2 n}{k} \cdot \frac{1}{a|W|} + 1$.

\begin{theorem}
\label{thm:SelectorsConstructive}
$\cS(n,\omega,k,c)$ is a $k$-light $(n,\omega)$-selector  of length 
$m = O\left (\min\{n,(\omega+n/k) \text{ polylog } n\}\right )$ for a sufficiently large constant $c$, and is constructed in time polynomial in $n$.
%\begin{gather}
%$    m = O\left (\omega \log n\right ) \mbox{   for  }   k \geq \frac{n}{\omega} \mbox{, and } 
%%    \nonumber\\ 
%    m = O\left (\frac{n}{k} \log n\right ) \mbox{  for   } k < \frac{n}{\omega}$.
%% \end{gather}
\end{theorem}

\begin{proof}
First we show that $\cS(n,\omega,k,c)$ is a $k$-light $(n,\omega)$-selector, for sufficiently large constant $c>0$.
%
First we consider more complex case of $n>a|W|\alpha$.
Let set $A\subseteq V$ be of size~between $\omega/2$ and $\omega$.
Suppose, to the contrary, that there are less than $\omega/4$ elements in $A$ hit by some sets in $\cS(n,\omega,k,c)$.
It implies that there is a subset $B\subseteq A$ of 
size $\omega/4+1$ such that none of the elements in~$B$
is hit by sets from $\cS(n,\omega,k,c)$.
%that is, $F(i)\cap A\ne \{v\}$,
%for each $v\in C$ and $1\le i\le m|W|$.

\noindent
\textsf{Claim:}
Every $w\in N_G(B)$ has more than 
$c\delta$ neighbors in~$A$, 
where $c\delta$ is a disjunctness parameter of $\cM$.
%for a sufficiently large constant $c$. 

The proof is by contradiction.
Assume, for simplicity of notation, that $w\in W$ 
is the $w$-th element of set~$W$.
Suppose, to the contrary, that
there is $w\in N_G(B)$ which has
at most $c\delta$ neighbors in~$A$,
that is, $|N_G(w)\cap A|\le c\delta$.
By the fact that $\cM$ is a $c\delta$-disjunct  
superimposed code, for $a=O((c\delta)^2 \log^2 n)$,
%$(n,c\delta\frac{k}{k-r+1})$-strongly-selective family 
we have that, for every $v\in N_G(w)\cap A$, the equalities
\[
F_{w\cdot a+y}\cap A = 
(M_y\cap N_G(w)) \cap A =
M_y\cap(N_G(w)\cap A) =
\{v\} 
\]
hold, for some $1\le y\le a$.
This holds in particular for every $v\in B\cap N_G(w)\cap A$.
There is at least one such~$v\in B\cap N_G(w)\cap A$, 
because set $B\cap N_G(w)\cap A$ is nonempty 
due to $w\in N_G(B)$ and $B\subseteq A$.
The existence of such~$v$ is in contradiction with the choice of set~$B$.
More precisely, $B$ contains only elements which are not hit
by sets from $\cS(n,\omega,k,c)$, but $v\in B\cap N_G(w)\cap A$ 
is hit by some set $F_{w\cdot a+y}$, thus is also hit by some children $S_j\in \cS(n,\omega,k,c)$ of $F_{w\cdot a+y}$.
This makes the proof of the Claim complete.

Recall that $|B|=\omega/4+1$.
By dispersion, the set $N_G(B)$ is of size larger than $(1-\ep)|W|$, 
hence, by the Claim above, the total number of edges 
between the nodes in $A$ and 
$N_G(B)$ in graph $G$ is larger than 
\[
(1-\ep)|W|\cdot c\delta = 
(1-\ep)\Theta((\omega/4+1)d/\delta) \cdot c\delta >
\omega d \ ,
\]
for a sufficiently large constant~$c$. 
This is a contradiction, since the total number of edges
incident to nodes in~$A$ is at most $|A|\cdot d=\omega d$. 
It follows that $\cS(n,\omega,k,c)$ is a $k$-light $(n,\omega,k)$-selector, for a sufficiently large constant $c$.

Before estimate the length $m$ of this selector, note that the union of all sets $F_j$ in the case $n> a|W|\alpha$
is at most $a\cdot (|V|\cdot d)$, because an element in some $F_j$ corresponds to some edge in the disperser
and repeats at most as many times as the number of rows $a$ in the superimposed code $\cM$.
Hence, the amortized number of children $S\in \cS(n,\omega,k,c)$ of a set $F_j$, parameter $\alpha$, is 
at most 
\[
\frac{a\cdot (|V|\cdot d)}{k} \cdot \frac{1}{a|W|} + 1 
%= 
%\frac{nd \cdot (c\delta)^2 \log^2 n}{k} + 1
\ .
\]

The length $m$ of this selector is thus at most
\begin{eqnarray*}
\min\{n,a|W|\alpha\} 
&=&
O\left(\min\left\{n,\delta^2\log^2 n\cdot
\omega d/\delta  + \frac{nd \cdot (c\delta)^2 \log^2 n}{k} \right\}\right)\\
&=&
O\left(\min\left\{n,(\omega + n/k)\polylog n\right\}\right)
\ ,
\end{eqnarray*}
since $d=O(\polylog n)$ and $\delta=O(\log^3 n)$.

The case $n\le a|W|\alpha$ is clear, since each element $i$ in a set~$A$ of
size~between $\omega/2$ and $\omega$ occurs as a singleton in some selector's set, mainly in~$S_i$.
\end{proof}



